NDST: Neural Driving Style Transfer for Human-Like Vision-Based Autonomous Driving

Autonomous Vehicles (AV) and Advanced Driver Assistant Systems (ADAS) prioritize safety over comfort. The intertwining factors of safety and comfort emerge as pivotal elements in ensuring the effectiveness of Autonomous Driving (AD). Users often experience discomfort when AV or ADAS drive the vehicle on their behalf. Providing a personalized human-like AD experience, tailored to match users' unique driving styles while adhering to safety prerequisites, presents a significant opportunity to boost the acceptance of AVs. This paper proposes a novel approach, Neural Driving Style Transfer (NDST), inspired by Neural Style Transfer (NST), to address this issue. NDST integrates a Personalized Block (PB) into the conventional Baseline Driving Model (BDM), allowing for the transfer of a user's unique driving style while adhering to safety parameters. The PB serves as a self-configuring system, learning and adapting to an individual's driving behavior without requiring modifications to the BDM. This approach enables the personalization of AV models, aligning the driving style more closely with user preferences while ensuring baseline safety critical actuation. Two contrasting driving styles (Style A and Style B) were used to validate the proposed NDST methodology, demonstrating its efficacy in transferring personal driving styles to the AV system. Our work highlights the potential of NDST to enhance user comfort in AVs by providing a personalized and familiar driving experience. The findings affirm the feasibility of integrating NDST into existing AV frameworks to bridge the gap between safety and individualized driving styles, promoting wider acceptance and improved user experiences.

==> 2_main/4_experimental_result.tex <==
\section{Experimental Results}
\label{sec:results}


In our experiments, various methods were used to verify that the NDST structure learns and personalizes the AV system by transferring the driver's driving style using a self-configuring PB.
In the training phase, the NDST structure was used to learn driving styles, Style A and Style B. During this process, the PBs learned the distribution of acceleration and deceleration control values associated with each driving style.
\input{fig/plot_style_gg_model}
The training results were evaluated by analyzing acceleration and deceleration outputs obtained from test track drives using PB1 and PB2, respectively. Subsequent verification confirmed the successful execution of the style transfer.
The result is seen in Fig.\ref{fig:plot_style_gg_model}, where Fig.\ref{fig:plot_style_gg_con} is a G-G diagram of the acceleration/deceleration results from PB1 which transferred Style A, and Fig.\ref{fig:plot_style_gg_agg} is a G-G diagram of the acceleration/deceleration results from PB2 which transferred Style B.
The difference between the two G-G diagrams clearly shows that the styles have been transferred successfully as each PB drove in a different style.
PB1 does not have a large change in acceleration so the area displayed on the G-G diagram is small. 
In contrast, PB2 \textcolor{teal}{(which transfers Style B) }%(transfer to Style B) 
has a large change in acceleration, almost 3 times the acceleration value compared to Style A transferred by PB1.


\input{fig/plot_style_testing}
\input{fig/distance_result_straight}
\input{fig/short_track}


Based on the results of driving on the test track, using 3D plot, the acceleration values for each road section were visualized. 
Fig.\ref{fig:plot_style_testing} is the result of visualizing these acceleration values.
Fig.\ref{fig:plot_styleA_testing} shows the result of driving on the test track in style A using the trained PB1, and Fig.\ref{fig:plot_styleB_testing} shows the result of driving on the same test track in style B using the trained PB2.
The target speed is set to 20 m/s and shows the vehicle accelerates from the starting point to reach the target speed. 
It then shows the car slowing down as it enters a curve and accelerating as it exits.
Although both PB1 and PB2 accelerate and decelerate to reach the target speed, the acceleration, and deceleration applied to reach that target speed are different.
Fig.\ref{fig:distance_result_straight} shows the velocity and control values of each model when the target speed is set on the straight road section.
Fig.\ref{fig:distance_result_straight_A} shows the driving data of the original dataset collected by driver 1 (top) and the PB1 (style A) driving data (bottom), and Fig.\ref{fig:distance_result_straight_B} shows the driving data of the original dataset collected by driver 2 (top) and the PB2 (style B) driving data (bottom). 
The PB1 (style A) took $2250 m$ from the starting point to reach $30 m/s$, but the PB2 (style B) reached $30 m/s$ in $500 m$, showing rapid acceleration and deceleration.
Also, since acceleration/deceleration values are higher in style B, we can see that the acceleration/deceleration periods of time are shorter in comparison with style A. This is obvious at the points of entering or exiting a curve road section.
In the curve section (Fig.\ref{fig:short_track}), both PB1 and PB2 slowed down from $20m/s$ to $15m/s$ before entering the curve, drove through the curve maintaining $15m/s$, and compared the acceleration and distance required by the two models to reach the target speed of $20m/s$ after escaping from the curve. 
PB2 (Style B) reached the target speed in $80m$, while PB1 traveled $150m$ to reach the target speed. 



==> 2_main/5_discussion.tex <==
\section{Disscussion}
\label{sec:guidelines}



==> fig/plot_style.tex <==
\begin{figure}[!t]
\centering
\includegraphics[width=1\columnwidth]{img/trained_style_plot.pdf}
\caption{A graph visualizing the change in acceleration and deceleration after driving on a test track. Blue = slow down, yellow = accelerate. \textcolor{magenta}{Display acceleration color on image} }
\label{fig:plot_style}
\end{figure}

==> fig/plot_style2.tex <==
\begin{figure}[!t]
    \centering
	  \subfigure[]{
	    \includegraphics[width=1\columnwidth]{img/conservative_model_style_plot.pdf}\label{fig:con_style_plot}
	    }
	  \newline
	  \subfigure[]{
	    \includegraphics[width=1\columnwidth]{img/aggressive_model_style_plot.pdf}\label{fig:agg_style_plot}
	    }
    \caption{
    (a) Conservative style.
    (b) Aggressive style.
    }
    \label{fig:plot_style2}
\end{figure}

==> fig/plot_style3.tex <==
\begin{figure}[thpb]
    \centering
    \subfloat[\label{fig:plot_style3_A}]{
	    \includegraphics[width=1\columnwidth]{img/conservative_style_plot.pdf}}    
	  \hfill
    \subfloat[\label{fig:plot_style3_B}]{
	    \includegraphics[width=1\columnwidth]{img/aggressive_style_plot.pdf}}
    \caption{
    (a) Style A driving data. (Left): Trained NDST model with PB1 driving on the test track, (Right): Dataset collected by driver 1 on the training track.
    (b) Style B driving data. (Left): Trained NDST model with PB2 driving on the test track, (Right): Dataset collected by driver 2 on the training track.
    }
    \label{fig:plot_style3}
\end{figure}




==> fig/short_track.tex <==
\begin{figure}[!tb]
\centering
\includegraphics[width=1\columnwidth]{img/short_track.pdf}
\caption{Acceleration/deceleration in curved sections
(a) Results from PB1 sending Style A.
(b) Results from PB2 sending Style B.
}
\label{fig:short_track}
\end{figure}
